Non-uniform Array and Frequency Spacing for Regularization-free Gridless DOA

Gridless direction-of-arrival (DOA) estimation with multiple frequencies can be applied in acoustics source localization problems. We formulate this as an atomic norm minimization (ANM) problem and derive an equivalent regularization-free semi-definite program (SDP) thereby avoiding regularization bias. The DOA is retrieved using a Vandermonde decomposition on the Toeplitz matrix obtained from the solution of the SDP. We also propose a fast SDP program to deal with non-uniform array and frequency spacing. For non-uniform spacings, the Toeplitz structure will not exist, but the DOA is retrieved via irregular Vandermonde decomposition (IVD), and we theoretically guarantee the existence of the IVD. We extend ANM to the multiple measurement vector (MMV) cases and derive its equivalent regularization-free SDP. Using multiple frequencies and the MMV model, we can resolve more sources than the number of physical sensors for a uniform linear array. Numerical results demonstrate that the regularization-free framework is robust to noise and aliasing, and it overcomes the regularization bias.

==> comment.tex <==
% As long as the temporal frequency separation was greater than a certain minimum separation, exact recovery of the active temporal frequencies was guaranteed. Furthermore, a semidefinite programming (SDP) framework that characterized the ANM problem was presented. 
% In \cite{chi2016guaranteed}, the author considered a super-resolution problem that had a similar setup to \cite{candes2014towards} except that the point spread function was assumed to be unknown. Based on the assumption that the point spread function was stationary and lived in a known subspace, the lifting trick was applied, and the problem was formulated using ANM. The model was generalized to non-stationary point spread functions in \cite{yang2016super}. 
% ANM for 2D temporal frequency estimation was studied in \cite{chi2014compressive}. In \cite{yang2015enhancing}, the authors proposed a reweighted ANM framework, which can enhance the sparsity and achieve super-resolution.  
% \begin{itemize}
%     \item \textbf{Regularization-based method} The SDP problem for the noisy and near collision case needs a carefully designed regularization (see \cite[eq. (21)]{wu2023gridless}). The noise regularization term requires prior knowledge of the noise power (the regularization hyperparameter $\eta$ is usually proportional to the noise power), and the performance may degrade significantly if the noise power estimation is inaccurate. In addition, the near collision regularization hyperparameter (associated with the $\ell_{1, 2}$ regularization) needs non-trivial fine-tuning. Although it turns out that $\lambda = k \cdot N_f$ ($N_f$ is the number of frequencies) gives a satisfactory performance in the empirical results, a great amount of effort to find an appropriate $k$ is needed. It is also worth mentioning that both noise and near collision regularization can potentially bring about bias, which will result in performance degradation. 
%     \item \textbf{Mostly for uniform frequency set} The method is mostly developed for the uniform frequency set. Although the fast algorithm for the non-uniform frequency set is proposed, there is no validation for the performance. 
%     \item \textbf{Sensitive to the end-fire sources in the noisy case} The method has trouble resolving the sources that are close to the end-fire in noisy cases. The noise may bring about ambiguities in the root-finding step and that will result in the wrap-around error in the DOA estimation.
%     \item \textbf{Inferior performance in the low SNR case} The empirical results in \cite{wu2023gridless} show that the method can outperform the competing method only if the signal-to-noise ratio (SNR) is high enough. Hence, the robustness to the noise achieved by the regularization is limited in the low SNR case.
%     \item \textbf{Demanding computational complexity and limited scalability} The method needs to solve a potentially large-scale SDP problem and it is computationally expensive. In practice, there may be a great number of frequencies, and it will bring about a demanding cost for the computation. 
    
% \end{itemize}


% The equivalent SDP framework proposed in \cite{wu2023gridless} is derived based on the dual atomic norm and is considered as the dual domain. The robustness to the noise is reflected as the regularization term in the SDP problem. 

% Before we introduce the MMV-MF model, we first overview the assumptions. 

% \subsection{Assumptions}
% The following assumptions are made for the array configuration and signal model:
% \begin{enumerate}
%     \item There are $N_m$ sensors forming a uniform linear array (ULA) with array spacing $d$.
%     \item There are $K$ active sources impinging on the array from unknown directions of arrival (DOAs) $\theta$.
%     \item Each source has $N_f$ active temporal frequency components, each at an integer multiple $f$ of a fundamental frequency $f_0$, i.e., $f \in \{1, \dots, N_f\}$ and $ff_0 \in \{f_0, \dots, N_ff_0\}$. This is only a technical assumption to simplify the analysis, and our method can be applied in any frequency set with the fast algorithm proposed in Sec. \ref{fast_ag}.
%     \item Suppose $d \leq \frac{c}{2f_0}$ holds (or, equivalently, $\frac{2\pi f_0d}{c} \leq \pi$),
%     % \footnote{The theory will first be derived based on the assumption $d = \frac{c}{2f_0}$. We will later see the theory will still hold when $d \leq \frac{c}{2f_0}$.} 
%     where $c$ is the speed of propagation. We also notice that $d = \frac{c}{2f_0}$ is the maximum separation to avoid spatial aliasing at the fundamental frequency. For higher frequencies (i.e. $f \geq 2$), aliasing will still exist. Such aliasing is not considered in conventional narrowband ANM papers. It is possible to develop the method with $d = \frac{c}{2N_ff_0}$ so that aliasing can be completely avoided in all frequencies. 
    
% \end{enumerate}

% \item Suppose $d = \frac{c}{2f_0}$ holds (or, equivalently, $\frac{2\pi f_0d}{c} \leq \pi$),
    % % \footnote{The theory will first be derived based on the assumption $d = \frac{c}{2f_0}$. We will later see the theory will still hold when $d \leq \frac{c}{2f_0}$.} 
    % where $c$ is the speed of propagation. We also notice that $d = \frac{c}{2f_0}$ is the maximum separation to avoid spatial aliasing at the fundamental frequency. For higher frequencies (i.e. $f \geq 2$), aliasing will still exist. Such aliasing is not considered in conventional narrowband ANM papers. It is possible to develop the method with $d = \frac{c}{2N_ff_0}$ so that aliasing can be completely avoided in all frequencies. 

% \subsection{Single Snapshot Case}
% \subsubsection{SDP in the Primal Domain}
% Assume $N_l = 1$ in this sub-section. The SDP in the primal domain is \cite[eq. (29)]{wu2023gridless}
% \begin{equation}
% \label{ssdp_dual_2}
% \begin{aligned}
%      \min_{\mathbf{W}, \mathbf{u}, \mathbf{\widetilde{Y}}} [\mathrm{Tr}(\mathbf{W}) + \mathrm{Tr(Toep}(\mathbf{u}))] \\
%     \quad \quad \textrm{s.t.} 
% \left[                 
%   \begin{array}{cc}   
%     \mathrm{Toep}(\mathbf{u}) & \mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H &  \mathbf{W}\\  
%   \end{array}
% \right]  \succeq 0, \mathbf{Y} = \mathcal{R}(\mathbf{\widetilde{Y}}),
% \end{aligned}
% \end{equation}
% where $\mathbf{W} \in \mathbb{C}^{N_f \times N_f}$, $\mathbf{u} \in \mathbb{C}^N$, and $\widetilde{\mathbf{Y}} \in \mathbb{C}^{N \times N_f}$.

% \subsubsection{Fast SDP Program}
% \label{fast_sdp}

% The dual problem is

% \begin{equation}
% \begin{aligned}
%      & \max_{\mathbf{W}, \mathbf{u}, \mathbf{\widetilde{Y}}} -\frac{1}{2}[\mathrm{Tr}(\mathbf{W}) + \mathrm{Tr(T}(\mathbf{u}))] \\
%     \quad & \textrm{s.t.} 
% \left[                 
%   \begin{array}{cc}   
%     \mathrm{T}(\mathbf{u}) & \mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H & \mathbf{W} \\  
%   \end{array}
% \right]  \succeq 0, \mathbf{Y} = \mathcal{R}_1(\mathbf{\widetilde{Y}}),
% \end{aligned}
% \end{equation}

% \begin{equation}
% \label{sdp_fast}
% \begin{aligned}
%      &\min_{\mathbf{W}, \mathbf{u}, \mathbf{\widetilde{Y}}} \mathrm{Tr}(\mathbf{W}) + \mathrm{Tr(T}(\mathbf{u})) \\
%     \quad  &\textrm{s.t.} 
% \left[                 
%   \begin{array}{cc}   
%     \mathrm{T}(\mathbf{u}) & \mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H & \mathbf{W} \\  
%   \end{array}
% \right]  \succeq 0, \mathbf{Y} = \mathcal{R}_1(\mathbf{\widetilde{Y}}),
% \end{aligned}
% \end{equation}

% \subsection{Multiple Snapshots Case}
% \subsubsection{SDP in the Primal Domain}
% Suppose $N_l > 1$, we can similarly derive the dual problem of \eqref{ssdp}. The dual problem is still an SDP, and it can expressed as 
% \begin{equation}
% \label{ssdp_dual_mmv}
% \begin{aligned}
%      &\min_{\mathbf{W}, \mathbf{u}, \mathbf{\widetilde{Y}}} [\mathrm{Tr}(\mathbf{W}) + \mathrm{Tr(Toep}(\mathbf{u}))] \\
%     \quad &\textrm{s.t.} 
% \left[                 
%   \begin{array}{cc}   
%     \mathrm{Toep}(\mathbf{u}) & \mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H &  \mathbf{W}\\  
%   \end{array}
% \right]  \succeq 0, \mathbf{Y}_f = \mathcal{R}(\mathbf{\widetilde{Y}}_f), (f = 1, \dots, N_f).
% \end{aligned}
% \end{equation}
% where $\mathbf{\widetilde{Y}} \in \mathbb{C}^{N \times N_lN_f}$, $\mathbf{Y}_f \in \mathbb{C}^{N_m \times N_l}$ is the $f$-th slice of the received signal tensor $\mathcal{Y}$, and $\mathbf{W} \in \mathbb{C}^{N_lN_f \times N_lN_f}$. We will apply this program in Sec. \ref{ula_source} to explore the possibility of resolving more sources than the number of sensors.

% \subsubsection{Fast SDP Program}
% Following the same procedure as Sec. \ref{fast_sdp}, we can obtain the fast SDP program in the MMV setup:
% \begin{equation}
% \label{ssdp_fast_mmv}
% \begin{aligned}
%      &\min_{\mathbf{W}, \mathbf{u}, \mathbf{\widetilde{Y}}} [\mathrm{Tr}(\mathbf{W}) + \mathrm{Tr(T}(\mathbf{u}))] \\
%     \quad &\textrm{s.t.} 
% \left[                 
%   \begin{array}{cc}   
%     \mathrm{T}(\mathbf{u}) & \mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H &  \mathbf{W}\\  
%   \end{array}
% \right]  \succeq 0, \mathbf{Y}_f = \mathcal{R}_1(\mathbf{\widetilde{Y}}_f), (f = 1, \dots, N_f).
% \end{aligned}
% \end{equation}
% where $\mathbf{\widetilde{Y}} \in \mathbb{C}^{N_u \times N_lN_f}$, $\mathbf{W} \in \mathbb{C}^{N_lN_f \times N_lN_f}$, $\mathbf{Y}_f \in \mathbb{C}^{N_m \times N_l}$ is the $f$-th slice of the received signal tensor $\mathcal{Y}$, and $\mathbf{\widetilde{Y}}_f \in \mathbb{C}^{N_u \times N_l}$ is taking $N_l$ columns from $\mathbf{\widetilde{Y}}$ ($(f - 1)\cdot N_l + 1$-th to $f \cdot N_l$-th column).


% In this section, we first overview a generalized version of the Vandermonde decomposition proposed in \cite{wagner2021} to facilitate us retrieving the DOAs from $\mathrm{T}(\mathbf{u})$ under the NUA or NUF case. Then, we explore the existence of the IVD for the fast algorithm proposed in Sec. \ref{fast}. We theoretically guarantee the existence of IVD that is not provided in \cite{wagner2021}.  

% \textit{Proof} Since $\mathrm{T}(\mathbf{u})$ is guaranteed to be a PSD matrix based on the constraints of \eqref{sdp_fast}, and its rank is $r$, it must exist the factorization such that $\mathrm{T}(\mathbf{u}) = \mathbf{VV}^H$, where $\mathbf{V} \in \mathbb{C}^{N_u \times r}$. Consider the rows of $\mathbf{V}$ as $\mathbf{V} = [\mathbf{v}_1, \dots, \mathbf{v}_{N_u}]^H$ (each row is denoted as $\mathbf{v}_i^H$). Then $\mathrm{T}(\mathbf{u})(i, j) = \mathbf{v}_i^H \mathbf{v}_j$. Notice that $\mathrm{T}(\mathbf{u})$ has identical diagonal elements (all equal to $\mathbf{u}_1$), therefore 
% \begin{equation}
%     \mathbf{v}_1^H \mathbf{v}_1 = \dots = \mathbf{v}_{N_u}^H \mathbf{v}_{N_u} = \mathbf{u}_1.
% \end{equation}

% According to \cite[Theorem 7.3.11]{horn2012matrix}, there must exist an $r \times r$ unitary matrix $\mathbf{Q}_i$ such that $\mathbf{v}_i = \mathbf{Q}_i \mathbf{v}_1$. \textbf{Can we show that $\mathbf{Q}_i = \mathbf{Q}^{\gamma_i - 1}$ ($\mathbf{Q}$ is a unitary matrix) ? We are certain that for each pair of $\mathbf{v}_i$ and $\mathbf{v}_j$, there exists a unitary matrix such that $\mathbf{v}_i = \mathbf{Q}_{ij} \mathbf{v}_j$, but how can we connect them to the power (maybe rational or irrational power) of a certain unitary matrix $\mathbf{Q}$? What I know is that any real power of the unitary matrix will be unitary, but I am not very sure how to apply the claim to get our desired results. }

% \textbf{To be specific, the math question we have to answer is: Suppose $\mathrm{T}(\mathbf{u}) \in \mathbb{C}^{N_u \times N_u}$ is a rank-$r$ PSD matrix with given entries defined in \eqref{T_map}, and its factorization is $\mathrm{T}(\mathbf{u}) = \mathbf{VV}^H (\mathbf{V} \in \mathbb{C}^{N_u \times r}). $ Consider each row of $\mathbf{V} = [\mathbf{v}_1, \dots, \mathbf{v}_{N_u}]^H$ (each row is denoted as $\mathbf{v}_i^H$), prove/disprove that $\mathbf{v}_i = \mathbf{Q}^{\gamma_i - 1} \mathbf{v}_1$, where $\mathbf{Q}$ is a unitary matrix, and $\gamma_i = \mathcal{U}_i + 1$ ($\gamma_i$ does not necessarily to be that value, as long as it is a real number, that shall be fine). }

% \textbf{There are some facts for the unitary matrix that can be helpful:
% \begin{itemize}
%     \item The eigenvalue decomposition of any unitary matrix always exists, and the amplitudes of all eigenvalues are 1.   
%     \item $\mathbf{v}_i^H \mathbf{v}_i = \mathbf{v}_j^H \mathbf{v}_j$ if and only if there exists a unitary matrix $\mathbf{Q}$ such that $\mathbf{v}_i = \mathbf{Qv}_j$
%     \item Any real power of the unitary matrix is unitary. (See the discussions in \\
%     \url{https://math.stackexchange.com/questions/3147548/is-real-power-of-unitary-matrix-unitary})
% \end{itemize}
% }

% For the unitary matrix $\mathbf{Q}$, its eigenvalue decomposition is guaranteed to exist and it can be expressed as
% \begin{equation}
%     \mathbf{Q} = \widetilde{\mathbf{Q}} \mathrm{diag}(z_1, \dots, z_r) \widetilde{\mathbf{Q}}^H,
% \end{equation}
% where $\widetilde{\mathbf{Q}}$ is unitary and $|z_1| = \dots = |z_r| = 1$. 

% Choose $z_k = e^{j2\pi w_k}$, $d_k = \|\widetilde{\mathbf{Q}}_{:k}^H \mathbf{v}_1\|_2^2$ and then
% \begin{equation}
%     \mathrm{T}(\mathbf{u})(i, j) = \mathbf{v}_i^H \mathbf{v}_j = \mathbf{v}_1^H \mathbf{Q}^{\gamma_j - \gamma_i} \mathbf{v}_1 = \sum_{k = 1}^r d_k z_k^{\gamma_j - \gamma_i}.
% \end{equation}

% Therefore, the decomposition in \eqref{van_decomp} is guaranteed to exist. 

% \begin{figure}[!t]
% \centering
% \includegraphics[width=8.5cm]{RMSE_SNR_N_f_2_15_165_1114.pdf}
% \caption{RMSE versus SNR when $N_f = 2$ with frequency set $\{100, 200\}$ Hz}
% \label{Nf_2}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=8.5cm]{RMSE_SNR_N_f_4_15_165_1114.pdf}
% \caption{RMSE versus SNR when $N_f = 4$ with frequency set $\{100, 200, 300, 400 \}$ Hz}
% \label{Nf_4}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=8.5cm]{RMSE_SNR_N_f_4_1235.pdf}
% \caption{RMSE versus SNR when $N_f = 4$ with frequency set $\{100, 200, 300, 500 \}$ Hz}
% \label{Nf_4_non_uniform}
% \end{figure}

% In addition to the RMSE in the angular domain, we also consider $\mathrm{RMSE}_u$, the RMSE in the $u = \cos(\theta)$ domain, defined as
% \begin{equation}
%     \mathrm{RMSE}_u = \sqrt{\frac{1}{MC} \sum_{m = 1}^{MC}\bigg[\frac{1}{K}\sum_{k = 1}^{K}(\cos(\hat{\theta}_{mk}) - \cos(\theta_{mk}))^2 \bigg]}.
% \end{equation}
% A maximum threshold of $0.2$ is used to compute the $\mathrm{RMSE}_u$.

% The ADMM algorithm can be unrolled based on ADMM-net. We will later explore the possibility of resolving endfire sources based on the ADMM unrolling network.

% \subsubsection{Deep Unrolling Network}
% Deep unrolling (or unfolding) \cite{monga2021algorithm, yang2016deep, yang2018admm, li2019algorithm, chen2021graph, sahel2022deep, zhu2022deep} has been proposed recently to connect iterative algorithms to deep neural networks that are both interpretable and generalizable. Gregor and LeCun developed this technique in their seminal work \cite{gregor2010learning} for the sparse coding problem. Following this work, there has been a surge of efforts to unroll iterative algorithms for many signal processing problems including  compressive sensing \cite{yang2016deep, yang2018admm, zhu2022deep}, deconvolution \cite{li2019algorithm}, graph signal processing \cite{chen2021graph}, and medical imaging \cite{sahel2022deep}. We refer readers to \cite{monga2021algorithm} for an overview of the recent progress in deep unrolling networks. 

%\textcolor{red}{More references about more sources than sensors, maybe see Piya Pal's introduction. }   \\

% \subsubsection{ADMM Implementation and Deep Unrolling Network} To reduce the computational complexity, we use the alternating direction method of multipliers (ADMM) \cite{boyd2011distributed}, an iterative method, to solve the SDP problem. Deep unrolling (or unfolding) networks \cite{monga2021algorithm} are recently proposed to combine model-based and data-driven methods. The deep unrolling network is based on an iterative algorithm and unrolls it to a number of layers that consist of learnable parameters. Most hyperparameters in the original iterative algorithm become the learnable parameters in the network. By feeding the network with training data, it can adjust these parameters properly to perform the task better.  Many works show that the deep unrolling network has a faster convergence compared to the original iterative method, better interpretability than black box neural networks, and satisfactory generalization performance in the data-limited case \cite{monga2021algorithm}. Moreover, with the help of training data, the unrolling network can potentially solve a more challenging task compared to the original iterative method. Due to such a benefit and the inspiration from \cite{yang2016deep, yang2018admm}, we unroll ADMM so that it can converge faster and resolve end-fire sources, one of the challenges in the DOA estimation. The proposed framework can solve a more challenging task and the complexity is greatly reduced so that the method can be applied to the practical case when numerous frequencies are present. 


% \section{Existence of Irregular Vandermonde Decomposition (IVD)}
% \label{IVD_exist}

% \begin{table}[]
%   \begin{center}    
%     \caption{\label{tab:table2} Summary of the SDPs in this work.}
%     \begin{tabular}{l|l|l|l|l} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
%      SDP  & Primal / Dual  & SMV / MMV & Uniform / Non-uniform  \\
%       \hline
%       \eqref{ssdp}/ \eqref{ssdp_noise} & Dual & MMV & Uniform  \\
%       \eqref{ssdp_nua} & Dual & MMV & Non-uniform  \\
%       \eqref{ssdp_fast_mmv} & Primal & MMV & Non-uniform \\
%       \eqref{ssdp_fast_smv} & Primal & SMV & Non-uniform  \\
%       \eqref{ssdp_mmv} & Primal & MMV & Uniform  \\          
%     \end{tabular}
%   \end{center}
% \end{table}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=8.5cm]{bar_chart_noise_free_fail.pdf}
% \caption{Histogram for the estimated DOAs for (a) ANM, and (b) SBL. $N_m = 4$, $N_f = 5$, $N_l = 20$, and $K = 12$. The true DOAs lie in $\{20^\circ, 30^\circ, 45^\circ, 60^\circ, 75^\circ, 85^\circ, 90^\circ, 105^\circ, 120^\circ, 135^\circ, 150^\circ, 165^\circ\}$. The RMSE for ANM is $9.3056^\circ$, and the RMSE for SBL is $7.1473^\circ$.}
% \label{hist_nf_fail}
% \end{figure}
 
% \begin{figure}[!t]
% \centering
% \includegraphics[width=8.5cm]{hist_more_source.pdf}
% \caption{Histogram for the estimated DOAs for (a) ANM, and (b) SBL. $N_m = 5$, $N_f = 5$, $N_l = 20$, SNR = $20$ dB, and $K = 6$. The true DOAs lie in $\{30^\circ, 60^\circ, 90^\circ, 105^\circ, 120^\circ, 150^\circ \}$. 100 trials are executed. The RMSE for ANM is $0.54^\circ$, and the RMSE for SBL is $2.60^\circ$.}
% \label{hist}
% \end{figure}

% Note $\mathrm{rank}(\mathbf{Z}_k) = 1$. We first introduce an important lemma for our further discussion. 
% \begin{lemma}
% \label{lemma_la}
%     Suppose $\mathbf{\widetilde{Y}} \neq \mathbf{0}$, and $\mathbf{B}:=\left[         
%   \begin{array}{cc}   
%     \mathbf{VDV}^H & \mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H & \mathbf{W} \\  
%   \end{array}
% \right] \succeq 0 $ ($\mathbf{VDV}^H$ is the Vandermonde decomposition of $\mathrm{Toep}(\mathbf{u})$), then $\mathbf{\widetilde{Y}}$ must lie in the range space of $\mathbf{V}.$
% \end{lemma}
% \textit{Proof} We prove by contradiction. Suppose $\mathbf{\widetilde{Y}}$ does not lie in the range space of $\mathbf{V}$, then $\mathbf{\widetilde{Y}} \in \mathcal{N}(\mathbf{V}^H)$ (i.e. $\mathbf{V}^H\mathbf{\widetilde{Y}} = \mathbf{0}$). Consider $\mathbf{U} := \left[                 
%   \begin{array}{cc}   
%     \mathbf{\widetilde{Y}} \\  
%     \mathbf{0} \\  
%   \end{array}
% \right]$, then $\mathbf{U}^H\mathbf{B}\mathbf{U} = \mathbf{\widetilde{Y}}^H \mathbf{VDV}^H \mathbf{\widetilde{Y}} = \mathbf{0}$.

% Since $\mathbf{B}$ is PSD, then $\mathbf{U}^H\mathbf{BU} = (\mathbf{B}^{1/2}\mathbf{U})^H\mathbf{B}^{1/2}\mathbf{U} = \mathbf{0}$ implies that $\mathbf{BU = 0}$. Thus, $\mathbf{BU} = \left[                
%   \begin{array}{cc}   
%     \mathbf{0} \\  
%     \mathbf{\widetilde{Y}}^H \mathbf{\widetilde{Y}} \\  
%   \end{array}
% \right] = \mathbf{0}$, and it implies $\mathbf{\widetilde{Y}} = \mathbf{0}$. This contradicts with our assumption $\mathbf{\widetilde{Y}} \neq \mathbf{0}$. Hence, $\mathbf{\widetilde{Y}}$ must lie in the range space of $\mathbf{V}$. $\hfill\square$


%
% First, we note that $\mathbf{\widetilde{Y}} \in \mathrm{range}(\mathbf{Z})$, where $\mathbf{Z} = [\mathbf{z}_1, \dots, \mathbf{z}_K] \in \mathbb{C}^{N_u \times K}$. The Vandermonde decomposition of $\mathrm{Toep}(\mathbf{u}) = \mathbf{ZDZ}^H$ leads to $\mathrm{range(Toep(\mathbf{u}) )}= \mathrm{range}(\mathbf{Z})$. Therefore, $\mathbf{\widetilde{Y}} \in \mathrm{range(Toep(\mathbf{u}))}$.
%
% Since $\mathrm{Toep}(\mathbf{u}^*)$ is a PSD matrix, we have $\mathbf{\widetilde{y}}^H \mathbf{VDV}^H \mathbf{\widetilde{y}} \geq 0 $ for any $\mathbf{\widetilde{y}} \in \mathbb{C}^{N_u}$. Now we consider $\mathbf{\widetilde{y}}$ as one of the columns of $\mathbf{\widetilde{Y}}$. Define $\mathbf{e} = \mathbf{V}^H \mathbf{\widetilde{y}}$. Therefore, $\mathbf{\widetilde{y}}^H \mathbf{VDV}^H \mathbf{\widetilde{y}} = \mathbf{e}^H \mathbf{D} \mathbf{e}$. Since $\mathbf{D}$ is also PSD, $\mathbf{e}^H \mathbf{D} \mathbf{e} \geq 0$ holds for any $\mathbf{e}$. We can conclude that $\mathbf{\widetilde{y}} \in \mathrm{range}(\mathbf{V})$. 

% In the proposition above, we choose one specific $\mathbf{\widetilde{Y}}$ based on \eqref{eq:ytildedef} so that the constraint in \eqref{ssdp_fast_smv} $\mathbf{Y} = \mathcal{R}(\widetilde{\mathbf{Y}})$ is satisfied. 

% (30) is searching for the Ytilde that has the smallest l0 norm while being consistent with the data, i.e., satisfying Y equals R of Ytilde.

% Prior works demonstrate that under a carefully designed array geometry (e.g., co-prime array), it is possible to resolve more sources than sensors. However, in the following example, we demonstrate that it is possible to resolve more sources than sensors under the ULA setup with the help of multiple frequencies.  In practice, ULA is frequently used because of its simplicity and in some cases, the array geometry may not be able to be changed. 

% \section*{ADMM and Deep Unrolling}
% \subsection{ADMM Update Equation Derivation}
% We start with the atomic norm denoising problem, which can be expressed as
% \begin{equation}
% \label{ssdp_dual_admm}
% \begin{aligned}
%      \min_{\mathbf{W}, \mathbf{u}, \mathbf{\widetilde{Y}}, \mathbf{Z}} \frac{1}{2}\|\mathbf{Y} - \mathcal{R}(\mathbf{\widetilde{Y}}) \|_F^2 + \frac{\tau}{2}[\mathrm{Tr}(\mathbf{W}) + \mathrm{Tr(Toep}(\mathbf{u}))] \\
%     \quad \quad \textrm{s.t.} \quad \mathbf{Z} = \left[                 
%   \begin{array}{cc}   
%     \mathrm{Toep}(\mathbf{u}) & \mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H &  \mathbf{W}\\  
%   \end{array}
% \right], \quad \mathbf{Z} \succeq 0, \quad \mathbf{Y} = \mathcal{R}(\mathbf{\widetilde{Y}}).
% \end{aligned}
% \end{equation}

% Then, the augmented Lagrangian is formed by collecting the constraints into the optimization function,
% \begin{equation}
% \label{Lagrange}
% \begin{aligned}
%     &\mathcal{L}(\mathbf{u}, \mathbf{W}, \widetilde{\mathbf{Y}}, \mathbf{Z}, \mathbf{\Lambda}, \mathbf{S}) = \frac{\tau}{2}\bigg[\mathrm{Tr}(\mathrm{Toep}(\mathbf{u})) + \mathrm{Tr}(\mathbf{W}) \bigg] + \\
%     &\bigg \langle \mathbf{\Lambda}, \mathbf{Z} \!\! - \!\! \left[                 
%   \begin{array}{cc}   
%     \mathrm{Toep}(\mathbf{u}) & \!\!\mathbf{\widetilde{Y}} \\  
%     \mathbf{\widetilde{Y}}^H &  \!\!\mathbf{W}\\  
%   \end{array}
% \right] \Bigg \rangle 
% + \frac{\rho_1}{2} \bigg \| \mathbf{Z}\!\!  - \!\!\left[                 
%   \begin{array}{cc}   
%     \!\!\mathrm{Toep}(\mathbf{u}) & \!\!\mathbf{\widetilde{Y}} \\  
%     \!\!\mathbf{\widetilde{Y}}^H &  \!\!\mathbf{W}\\  
%   \end{array}
% \right] \Bigg \|_F^2 \\
% + &\langle \mathbf{S}, \mathbf{Y} - \mathcal{R}(\widetilde{\mathbf{Y}}) \rangle + \frac{\rho_2 + 1}{2} \| \mathbf{Y} - \mathcal{R}(\widetilde{\mathbf{Y}}) \|_F^2
% \end{aligned}
% \end{equation}
% where $\rho_1$, $\rho_2$ are user defined parameters. $\mathbf{\Lambda}$, and $\mathbf{S}$ are Lagrange multipliers. ADMM aims to iteratively optimize \eqref{Lagrange} over each variable. The update steps at iteration $n$ are
% \begin{equation}
%     (\mathbf{u}^{(n + 1)}, \mathbf{W}^{(n + 1)}, \mathbf{\widetilde{Y}}^{(n + 1)}) \leftarrow \mathrm{argmin}_{\mathbf{u},\! \mathbf{W},\! \widetilde{\mathbf{Y}}} \mathcal{L}(\mathbf{u},\! \mathbf{W},\! \widetilde{\mathbf{Y}},\! \mathbf{Z}^{(n)},\! \mathbf{\Lambda}^{(n)},\! \mathbf{S}^{(n)})
% \end{equation}

% \begin{equation}
%     \mathbf{Z}^{(n + 1)} \leftarrow \mathrm{argmin}_{\mathbf{Z} \succeq 0} \mathcal{L}(\mathbf{u}^{(n+1)},\! \mathbf{W}^{(n+1)},\! \widetilde{\mathbf{Y}}^{(n+1)}, \! \mathbf{Z}, \! \mathbf{\Lambda}^{(n)}, \! \mathbf{S}^{(n)})
% \end{equation}

% \begin{equation}
% \label{Lambda_update}
%     \mathbf{\Lambda}^{(n+1)} \leftarrow \mathbf{\Lambda}^{(n)} + \eta_1 \Bigg (\mathbf{Z}^{(n+1)} - \left[
%   \begin{array}{cc}   
%     \mathrm{Toep}(\mathbf{u}^{(n+1)}) & \mathbf{\widetilde{Y}}^{(n+1)} \\  
%     \mathbf{\widetilde{Y}}^{(n+1) H} &  \mathbf{W}^{(n+1)}\\  
%   \end{array}
% \right] \Bigg)
% \end{equation}


% \begin{equation}
% \label{S_update}
%     \mathbf{S}^{(n+1)} \leftarrow \mathbf{S}^{(n)} + \eta_2 [\mathbf{Y} - \mathcal{R}(\mathbf{\widetilde{Y}}^{(n+1)})]
% \end{equation}

% Note for standard ADMM, $\eta_1 = \rho_1$ and $\eta_2 = \rho_2$ in \eqref{Lambda_update} and \eqref{S_update}. To increase the capacity the of the unrolling network developed in the following section, we change them to $\eta_1$ and $\eta_2$.

% The update steps for $\mathbf{u}$, $\mathbf{W}$, $\widetilde{\mathbf{Y}}$, $\mathbf{Z}$ can be expressed in closed form. Define the partitions
% \begin{equation}
%     \mathbf{Z}^{(n)} = \left[
%   \begin{array}{cc}   
%     \mathbf{Z}_{\mathbf{u}}^{(n)} & \mathbf{Z}_{\widetilde{\mathbf{Y}}}^{(n)} \\  
%     \mathbf{Z}_{\widetilde{\mathbf{Y}}^H}^{(n)} &  \mathbf{Z}_{\mathbf{W}}^{(n)}\\  
%   \end{array}
% \right], \quad \mathbf{\Lambda}^{(n)} = \left[
%   \begin{array}{cc}   
%     \mathbf{\Lambda}_{\mathbf{u}}^{(n)} & \mathbf{\Lambda}_{\widetilde{\mathbf{Y}}}^{(n)} \\  
%     \mathbf{\Lambda}_{\widetilde{\mathbf{Y}}^H}^{(n)} &  \mathbf{\Lambda}_{\mathbf{W}}^{(n)}\\  
%   \end{array}
% \right]
% \end{equation}
% where the dimensions of each partition are the dimensions of $\mathrm{Toep}(\mathbf{u})$, $\widetilde{\mathbf{Y}}$, and $\mathbf{W}.$ The update steps can be summarized as:
% \begin{equation}
% \label{W_update}
%     \mathbf{W}^{(n+1)} = \frac{1}{2} \bigg(\mathbf{Z}_{\mathbf{W}}^{(n)} + \mathbf{Z}_{\mathbf{W}}^{(n) H} \bigg) + \frac{1}{\underline{\rho_1}} \bigg(\mathbf{\Lambda}_{\mathbf{W}}^{(n)} - \frac{\underline{\tau}}{2}\mathbf{I} \bigg)
% \end{equation}


% \begin{equation}
% \label{u_update}
%     \mathbf{u}^{(n+1)} = \underline{\mathrm{Toep}}^{-1} \bigg(\mathbf{Z}_{\mathbf{u}}^{(n)} + \frac{1}{\underline{\rho_1}} \mathbf{\Lambda}_{\mathbf{u}}^{(n)} \bigg) - \frac{\underline{\tau}}{2\underline{\rho_1}}\mathbf{e}_1
% \end{equation}

% \begin{equation}
% \begin{aligned}
% \label{Y_tild_update}
%     \widetilde{\mathbf{Y}}^{(n+1)} &= \frac{1}{2\underline{\rho_1} + \underline{\rho_2} + 1} \bigg( \mathbf{\Lambda}_{\widetilde{\mathbf{Y}}}^{(n)} + \mathbf{\Lambda}_{\widetilde{\mathbf{Y}}^H}^{(n)H}  + \underline{\rho_1}(\mathbf{Z}_{\widetilde{\mathbf{Y}}}^{(n)} + \mathbf{Z}_{\widetilde{\mathbf{Y}}^H}^{(n)H}) \\
%     &+ \mathcal{R}^*(\mathbf{S}^{(n)}) + \underline{\rho_2} \mathcal{R}^{*}(\mathbf{Y}) \bigg)
% \end{aligned}
% \end{equation}

% where $\mathrm{Toep}^{-1}$ is an operator that gives the first column of the nearest Toeplitz matrix to its input. $\mathbf{e}_1$ is the $N$-dimensional canonical basis $[1 \quad 0 \quad \dots \quad 0]^T$. 

% Finally, the $\mathbf{Z}$ update is a projection onto the positive semi-definite cone 
% \begin{equation}
% \label{Z_update}
%     \mathbf{Z}^{(n + 1)} = P_{\mathbf{Z} \succeq 0 } \Bigg ( \left[
%   \begin{array}{cc}   
%     \mathrm{Toep}(\mathbf{u}^{(n+1)}) & \mathbf{\widetilde{Y}}^{(n+1)} \\  
%     \mathbf{\widetilde{Y}}^{(n+1) H} &  \mathbf{W}^{(n+1)}\\  
%   \end{array}
% \right] - \frac{1}{\underline{\rho_1}} \mathbf{\Lambda}^{(n)} \Bigg).
% \end{equation}


% From the implementation point of view, the update equations can be executed with the following order \eqref{W_update} $\rightarrow$ \eqref{u_update} $\rightarrow$ \eqref{Y_tild_update} $\rightarrow$ \eqref{Z_update} $\rightarrow$ \eqref{Lambda_update} $\rightarrow$ \eqref{S_update}. Note that the performance of ADMM is sensitive to the hyperparameters $\{\rho_1, \rho_2, \eta_1, \eta_2, \tau\}$ which need to be fine-tuned. In addition, ADMM is shown to converge slowly. We will explore the ADMM unrolling network to speed up the convergence rate and make the hyperparameters learnable from the data. The learnable parameters and mappings in \eqref{Lambda_update} - \eqref{Z_update} are underlined. 


% \subsection{ADMM Unrolling Network}
% \subsubsection{Network Architecture}
% The proposed ADMM unrolling network aims to learn the hyperparameters and some of the linear maps in the ADMM update equations. The unrolling network maps the $L$ iterations in the original ADMM algorithm to $L$ layers. The learnable parameters are $\mathbf{\Omega} = \{\rho_1^{(l+1)}, \rho_2^{(l+1)}, \eta_1^{(l+1)}, \eta_2^{(l+1)}, \tau^{(l+1)}\}_{l = 0}^{ - 1}$, and the learnable map is $\mathrm{Toep}^{-1}$. The $(l + 1)$-th layer operation of the unrolling network can be expressed as 
% \begin{equation}
%     [\mathbf{u}^{(l + 1)}, \mathbf{Z}^{(l + 1)}, \mathbf{\Lambda}^{(l + 1)}, \mathbf{S}^{(l + 1)}] = F_{l + 1}\{\mathbf{Y}, \mathbf{Z}^{(l)}, \mathbf{\Lambda}^{(l)}, \mathbf{S}^{(l)} \}
% \end{equation}
% where $F_{l + 1}$ is the operation for the $(l + 1)$-th layer. The architecture of the unrolling network can be shown in Fig. \ref{Unroll_net}, and the data flow of each layer is detailed in Fig. \ref{Unroll_net2}.

% The network is trained in a supervised way and the ground truth $\mathbf{u}^{gt}$ is generated by CVX by solving a noise-free SDP problem. The output of the network is $\mathbf{u}^{(L)}$ and the loss function is 
% \begin{equation}
%     L = \bigg\| \frac{\mathbf{u}^{(L)}}{\| \mathbf{u}^{(L)}\|_2} - \frac{\mathbf{u}^{gt}}{\| \mathbf{u}^{gt} \|_2} \bigg\|_2.
% \end{equation}


% \begin{figure}[t]
% \centering
% \includegraphics[width=8.5cm]{Unroll_net_flow-1.pdf}
% \caption{Unrolling network architecture}
% \label{Unroll_net}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=8.5cm]{Unroll_net_flow-2.pdf}
% \caption{Details for $F_l\{\cdot\}$}
% \label{Unroll_net2}
% \end{figure}

% \subsection{ADMM Unrolling Performance Study}
% In this section, we test the performance of the unrolling network. The network is trained for 25 epochs. The learning rate is 0.001. For the dataset, 80\% is used for training and 20\% is used for validation. We unroll the $\mathrm{Toep}^{-1}$ operator as a series of convolutional layers (kernel size 3, stride 1, and padding 1) with ReLu activation functions. 



% \subsubsection{Testing Performance}
% In this section, we compare the performance of the deep unrolling network with SBL and ADMM. All of the methods are tested under the following setup: $N_m = 16$, $N_f = 1, 2, 4$, white noise is added and SNR = $10$ dB, and $K = 3$ sources randomly generated from $[0^\circ, 180^\circ]$. Therefore, the sources can be from the endfire region. The $20$-layer unrolling network plays the same role as ADMM with $20$ iterations. Therefore, its performance is compared to ADMM with $20$ iterations. The unrolling network is initialized with the same parameters ($\{\rho_1, \rho_2, \eta_1, \eta_2, \tau\}$) as ADMM. We notice that ADMM may achieve a better performance when more iterations are executed. Therefore, ADMM with $1500$ iterations are also included in the comparison. Fig. \ref{unroll_rmse} (a) - (b) demonstrates the superior performance of the unrolling network over ADMM with the same number of iterations and SBL with $0.1^\circ$ grid resolution \cite{nannuru2019sparse}. The unrolling network can outperform ADMM with $1500$ iterations in some cases while saving a great amount of running time as shown in Fig. \ref{gpu_time}.    

% \subsubsection{Generalization Performance}
% In this section, we will test the generalization performance of the unrolling network. The network will be tested with a different number of sources (2 sources) than the training data (3 sources). Note that for ADMM, SBL, and the proposed unrolling network, prior knowledge of the number of sources is required as part of the input to the method, while ADMM and SBL do not require a training process. From Fig. \ref{unroll_rmse} (c) - (d), the network generalizes to a different number of sources and outperforms the baseline method SBL. 

% In addition, we consider the generalization performance when one source is located close to the endfire. We generate $3$ sources and one source is fixed in $160^\circ$ (close to the endfire), and the rest 2 sources are randomly generated between $[30^\circ, 150^\circ]$. Fig. \ref{unroll_endfire} shows that the performance of the unrolling network does not significantly degrade in this case, which demonstrates the unrolling network is able to resolve endfire sources, a challenging case in the DOA estimation. 

% \begin{figure}[!t]
% \centering
% \includegraphics[width=8.5cm]{bar_chart_2plot.pdf}
% \caption{RMSE ($^\circ$) and u-RMSE comparison for the ADMM (20/1500 iterations), unrolling Network, and SBL. (a) There are $K = 3$ sources for both training and testing data. (b) There are 3 sources for training data and 2 sources for testing data. SNR = 10 dB for all cases.}
% \label{unroll_rmse}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=6cm]{bar_chart_gen_endfire.pdf}
% \caption{RMSE ($^\circ$) for the endfire source case. Note ``unroll'' is the same as Fig. \ref{unroll_rmse}. $K = 3$. One source is fixed in $160^\circ$, and the rest 2 sources are randomly generated between $[30^\circ, 150^\circ]$. }
% \label{unroll_endfire}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=6cm]{GPU_time.pdf}
% \caption{Running time comparison for Fig. \ref{unroll_rmse} (a) - (b)}
% \label{gpu_time}
% \end{figure}

%Each source has $N_f$ active temporal frequency components, and the frequency set is $\{F_1, \dots, F_{N_f}\}$. We assume frequencies are ascending but they might not be uniformly spaced. The wavelength set is therefore $\{\lambda_1, \dots, \lambda_{N_f}\} = \{c/F_1, \dots, c/F_{N_f}\}$. 

%There are $N_m$ sensors forming an array with sensor spacing unit $d = \frac{\lambda_1}{2} = \frac{c}{2F_1}$  and the sensors are located in $\{ M_1, \dots, M_{N_m}\} \cdot d$, where $M_1, \dots, M_{N_m}$ are real numbers sorted in ascending order and they may not be uniformly spaced.  
%Suppose the array is a ULA with sensor spacing $d$ and the frequencies are uniform (i.e., the sensor position set is $\{0, \dots, N_m - 1\} \cdot d$, and the frequency set is ${\{1, \dots, N_f\} \cdot F_1}$). 

%An irregular Vandermonde matrix $\mathbf{W}(\bm{\gamma}, \mathbf{z}) \in \mathbb{C}^{N_u \times K}$ ($N_u$ is the dimension of $\bm{\gamma}$, and it includes all possible exponents of $z$ in $\mathbf{a}(f, w)$ for $f = 1, \dots, N_f$. We will discuss its physical meaning in Sec. \ref{nua_nuf}) has the following structure 

% For the ULA and single-frequency case, $\bm{\gamma}$ becomes a progression of integers,  $\bm{\gamma} = [0, \dots, N_m - 1]^T$, $\mathbf{W}(\bm{\gamma}, \mathbf{z})$ is a regular Vandermonde matrix, and $\mathbf{T}$ is a regular Toeplitz matrix with a regular Vandermonde decomposition. 



% KEEPING A BACKUP OF SECTION II-D and II-E
%\subsection{Irregular Vandermonde and Toeplitz Matrices}
%\label{Irregular}
%An irregular Vandermonde matrix $\mathbf{W}(\bm{\gamma}, \mathbf{z}) \in \mathbb{C}^{N_u \times K}$ ($N_u$ is the dimension of $\bm{\gamma}$, and it includes all possible exponents of $z$ in $\mathbf{a}(f, w)$ for $f = 1, \dots, N_f$. We will discuss its physical meaning in Sec. \ref{nua_nuf}) has the following structure \cite[eq. (25)]{wagner2021}
%\begin{equation}
%    \mathbf{W}(\bm{\gamma}, \mathbf{z}) = [\mathbf{z}^{\gamma_1}, \dots, \mathbf{z}^{\gamma_{N_u}}]^T = [\mathbf{w}(\bm{\gamma}, z_1), \dots, \mathbf{w}(\bm{\gamma}, z_K)],
%\end{equation}
%where $\gamma_i$ is the $i$th element of $\bm{\gamma} \in \mathbb{R}^{N_u}$, $\mathbf{z} = [z_1, \dots, z_K]^T \in \mathbb{C}^K$, and $\mathbf{w}(\bm{\gamma}, z) = [z^{\gamma_1}, \dots, z^{\gamma_{N_u}}]^T$. 
%
%An irregular Toeplitz matrix $\mathbf{T} \in \mathbb{C}^{N_u \times N_u}$~\cite[eq. (27)]{wagner2021} is defined to be any matrix that can be constructed from an irregular Vandermonde matrix as follows:
%\begin{equation}
%\label{IV}
%    \mathbf{T} = \mathbf{W}(\bm{\gamma}, \mathbf{z})\mathbf{D} \mathbf{W}(\bm{\gamma}, \mathbf{z})^H, |\mathbf{z}| = 1
%\end{equation}
%where $\mathbf{D} \in \mathbb{R}^{K \times K}$ is a diagonal matrix. We refer to~\eqref{IV} as an irregular Vandermonde decomposition (IVD). 
%
%
%For the ULA and single-frequency case, $\bm{\gamma}$ becomes a progression of integers,  $\bm{\gamma} = [0, \dots, N_m - 1]^T$, $\mathbf{W}(\bm{\gamma}, \mathbf{z})$ is a regular Vandermonde matrix, and $\mathbf{T}$ is a regular Toeplitz matrix with a regular Vandermonde decomposition. 
%
%\subsection{IVD and DOA Extraction}
%\label{IVD_DOA}
%In Sec. \ref{Irregular}, we see that the DOA information is encoded in the irregular Vandermonde matrix $\mathbf{W}(\bm{\gamma}, \mathbf{z})$ that can be obtained by the IVD of $\mathbf{T}$. In this section, we will discuss how to extract the DOA based on IVD.
%
%Suppose $\mathbf{T} \in \mathbb{C}^{N_u \times N_u}$ is an irregular Toeplitz matrix with decomposition as in~\eqref{IV} with $\mathbf{z} \in \mathbb{C}^K$ that contains the information of $K$ DOAs, and consider the eigen-decomposition of $\mathbf{T}$:
%\begin{equation}
%    \mathbf{T} = \mathbf{U}_S \mathbf{\Lambda}_S \mathbf{U}_S^H + \mathbf{U}_N \mathbf{\Lambda}_N \mathbf{U}_N^H,
%\end{equation}
%where $\mathbf{\Lambda}_S \in \mathbb{C}^{K \times K}$ is a diagonal matrix containing the $K$ largest eigenvalues of $\mathbf{T}$, $\mathbf{U}_S \in \mathbb{C}^{N_u \times K}$ contains the corresponding eigenvectors, and $\mathbf{\Lambda}_N \in \mathbb{C}^{(N_u - K) \times (N_u - K)}$ and $\mathbf{U}_N \in \mathbb{C}^{N_u \times (N_u - K)}$ contain the remaining (zero) eigenvalues and corresponding eigenvectors. $\mathbf{U}_S$ and $\mathbf{U}_N$ are known as the \textit{signal and noise subspaces}, respectively. 
%
%The irregular null spectrum of $\mathbf{T}$ is \cite[eq. (29)]{wagner2021}
%\begin{equation}
%\label{D_z}
%    \Tilde{D}(z) = \mathbf{w}(\bm{\gamma}, z)^H \mathbf{U}_N \mathbf{U}_N^H \mathbf{w}(\bm{\gamma}, z) = \mathbf{w}(\bm{\gamma}, z)^H \mathbf{G} \mathbf{w}(\bm{\gamma}, z), 
%\end{equation}
%where $\mathbf{G} = \mathbf{U}_N \mathbf{U}_N^H$. The behavior of the irregular null spectrum is plotted in Fig. \ref{null_spec}. 
%
%Since $\mathbf{G} \perp \mathbf{W}(\bm{\gamma}, \mathbf{z})$ and $|z|  = 1$, the DOAs encoded in $\mathbf{z}$ are associated to the $K$ roots of $\Tilde{D}(z)$ on the unit circle. \cite{wagner2021} suggests that the local minima of $\Tilde{D}(z)$ evaluated on the unit circle give DOA estimates with similar accuracy as those given by the actual roots. Therefore, $\mathbf{z}$ is estimated as \cite[eq. (43)]{wagner2021}
%\begin{equation}
%   \hat{\mathbf{z}} = \mathrm{arg} \min_{|z| = 1}^k \Tilde{D}(z), \quad k = 1, \dots, K
%\end{equation}
%where $\mathrm{arg} \min_z^k$ denotes the argument, $z$, which produces the $k$th smallest local minima. The DOAs $\hat{\theta}, \hat{w},$ and $\hat{z}$ are estimated by
%\begin{equation}
%\hat{\theta} = \cos^{-1}\bigg(-\frac{\angle \hat{z}}{\pi} \bigg), \quad
%\hat{w} = \frac{-\angle \hat{z}}{2 \pi}, \quad
%\hat{z} = e^{-j \pi \cos(\hat{\theta})}.
%\end{equation}

%Recall that in the ULA case, the sensor position set is $\{0, \dots, N_m - 1\} \cdot d$. We model the NUA case by assuming the sensors are positioned at a subset of points from this set. We let $\mathcal{M} \subseteq \{0, \dots, N_m - 1\}$ denote the indices of the sensors in the NUA; the resulting positions are thus $\{m \cdot d|m \in \mathcal{M}\}$. Similarly, in the uniform frequency case, the frequency set is ${\{1, \dots, N_f\} \cdot F_1}$. We model the NUF case by assuming the frequencies are a subset of this set. We let $\mathcal{F} \subseteq \{1, \dots, N_f\}$ denote the indices; the resulting nonuniform frequencies are thus $\{f \cdot F_1|f \in \mathcal{F}\}$. The cardinalities $|\mathcal{M}| \le N_m$ and $|\mathcal{F}| \le N_f$ denote the number of nonuniform sensors and frequencies, respectively. When $|\mathcal{M}| = N_m$ and $|\mathcal{F}| = N_f$, respectively, we recover the uniform cases.

%We assume the $N_m$ sensors are positioned at points on a line given by spatial index set $\mathcal{M} = \{M_1, M_2, \dots, M_{N_m}\} $, and the normalized frequency index set is $\mathcal{F} = \{1, F_2/F_1, \dots, F_{N_f}/F_1\} $ (recall that the unnormalized frequency set is $\{F_1, F_2,\dots, F_{N_f}\}$). Note that for the ULA, $\mathcal{M} = \{0, 1, \dots , (N_m - 1)\}$, and for uniform frequencies, $\mathcal{F} = \{1, 2, \dots, N_f\} \cdot F_1$. In this section, we generalize the SDP to the NUA and NUF cases where neither $\mathcal{M}$ nor $\mathcal{F}$ is an arithmetic progression. 

%The generalized array manifold vector at frequency $F_f$ is 
%\begin{equation}
%\begin{aligned}
%     \mathbf{a}(F_f, w) &= [e^{-j2\pi w F_f/F_1 M_1} \dots e^{-j2\pi w F_f/F_1 M_{N_m}}]^T \\
%     &= [e^{-j2\pi d \cos(\theta)/c \cdot F_f M_1} \dots e^{-j2\pi d \cos(\theta)/c \cdot F_f M_{N_m}}]^T.
%\end{aligned}
%\end{equation}

% \textbf{Remark 4} $\mathbf{\widetilde{Y}}$ has $N_u$ rows and can be interpreted as a measurement matrix in the $\mathcal{U}$ domain

% Note to self: here is the story we want to tell. 
% 1. While problem (23) comes from taking the dual of (18), it has an interesting connection to the SDPs from the ANM literature which involve trace minimization of a regular Toeplitz matrix. Non-fast version of (23) (essentially (25)) has Toep(u) and R instead of R1. In (23), we have trace minimization of an irregular Toeplitz matrix. 
% 2. In ANM problems which involve trace minimization of a regular Toeplitz matrix, one typically computes the Vandermonde decomposition of the resulting Toeplitz matrix in order to extract the frequencies/DOAs. Based on the fact that an IVD exists (Thm 4.1) and insight from the IVD (Section IV-F), we propose to use the irregular null spectrum of the irregular Toeplitz matrix to recover the DOAs.
% 3. [UNDER CONSTRUCTION] In the UA/UF (or possibly non-fast) case, we motivate this by making a connection with atomic L0 minimization in Prop 6.1. (By the way, does that proposition then exactly match Theorem 11.13 in Zai Yang's book?)
% 4. In the NUF/NUA/fast case, we don't have all of the entries of Y, but we interpret it as a search for a low-rank Toeplitz matrix that is consistent with what is observed. Experimentally this works out well.

%and has the following IVD:
%\begin{equation}
%\label{van_decomp}
%    \mathrm{T}(\mathbf{u}) = \mathbf{G}(\bm{\gamma}, \mathbf{z}) \mathbf{D} \mathbf{G}(\bm{\gamma}, \mathbf{z})^H = \sum_{k = 1}^r d_k \mathbf{g}(\bm{\gamma}, z_k) \mathbf{g}(\bm{\gamma}, z_k)^H
%\end{equation}
%where 
%\begin{equation}
%\begin{aligned}
%    r &= \mathrm{rank}(\mathrm{T}(\mathbf{u})) \leq N_u \\
%    \mathbf{D} &= \mathrm{diag}(d_1, \dots, d_r) \\
%    \mathbf{G}(\bm{\gamma}, \mathbf{z}) &= [\mathbf{g}(\bm{\gamma}, z_1) \dots \mathbf{g}(\bm{\gamma}, z_r)] (\bm{\gamma} = [\mathcal{U}_1, \dots, \mathcal{U}_{N_u}]^T) \\
%    \mathbf{g}(\bm{\gamma}, z_k) &= [z^{\mathcal{U}_1}_k, \dots, z^{\mathcal{U}_{N_u}}_k]^{T}.
%\end{aligned}
%\end{equation}

\begin{comment}
Define $\Omega$ as the index set that includes all entries in $\mathbf{v}$ that appear in $\mathrm{T}(\mathbf{v})$ (these entries are called ``non-free'' entries). Entrywise, this IVD gives $\mathrm{T}(\mathbf{v}) (i, j) = \sum_{k = 1}^K d_k z_k^{\mathcal{U}_i - \mathcal{U}_j} $. Comparing to \eqref{T_map}, then, the entries in the set $\Omega$  and the entries of $\mathbf{W}$ and $\mathbf{D}$ must agree as follows:
\begin{equation}
 v_i = \sum_{k = 1}^K d_k z_k^{-i} , \quad   (i \in \Omega),
\end{equation}
or equivalently,
\begin{equation}
\mathbf{v}_{\Omega} = \mathbf{W}_{\Omega}(\bm{\gamma}, \mathbf{z}) [d_1, \dots, d_K]^T,
\end{equation}
where $\mathbf{v}_{\Omega} \in \mathbb{C}^{|\Omega|}$ and $\mathbf{W}_{\Omega} \in \mathbb{C}^{|\Omega| \times K}$ are projections of $\mathbf{v}$ and $\mathbf{W}$ to the index set $\Omega$.
\end{comment}

%As discussed further in Section~\ref{fast}, in this paper we propose an SDP whose output is an irregular Toeplitz matrix, and by performing an IVD on this irregular Toeplitz matrix, the DOAs can be estimated. Key to this connection is that the vector $\mathbf{z}$ in this decomposition will have dimension $K$, where $K$ is the number of active sources, and each entry of $\mathbf{z}$ will encode the DOA of one source. In this section, we discuss how to extract the DOAs from the IVD.

% Setting $N_\gamma = N_u$, the dimension defined and used in \eqref{ssdp_fast_mmv}, 

% However, $\eqref{cov_est}$ cannot be simply computed via the measurement data $\mathbf{Y}$ and we need to solve the optimization problem (e.g. \eqref{ssdp_fast_smv}) to obtain $\mathbf{\widetilde{Y}}$ and $\mathrm{Toep}(\mathbf{u})$ ($\mathrm{Toep}(\mathbf{u})$ can be interpreted as the covariance matrix). 

%
% We will first define the atomic $\ell_0$ norm and then show that minimizing the atomic $\ell_0$ norm essentially minimizes the rank of the estimated covariance matrix. Since the atomic norm is the convex relaxation of the atomic $\ell_0$ norm, the low-rank structure is also promoted in the ANM optimization problem.

\textit{Proof} The case for $\mathbf{\widetilde{Y}} = \mathbf{0}$ is trivial as we can choose $\mathbf{u} =  \mathbf{0}$, $\mathbf{W} = \mathbf{0}$, and $\mathrm{rank}(\mathrm{Toep}(\mathbf{u})) = \|\mathbf{\widetilde{Y}} \|_{\mathcal{A}, 0} = 0$.

If $\mathbf{\widetilde{Y}} \neq \mathbf{0}$, denote $\mathbf{u}^*$ as the optimal solution for \eqref{rank_min}, $r^* = \mathrm{rank(Toep}(\mathbf{u}^*))$, and $s = \|\mathbf{\widetilde{Y}} \|_{\mathcal{A}, 0}$. We have to show $r^* = s$. 

We begin with showing $r^* \leq s$. Suppose the atomic decomposition $\mathbf{\widetilde{Y}} = \sum_{k = 1}^K c_k \mathbf{z}_k \mathbf{x}_k^H$ with $c_k > 0$ achieves $\|\mathbf{\widetilde{Y}} \|_{\mathcal{A} , 0}$ (i.e. $K = s$). Set $\mathrm{Toep}(\mathbf{u}) = \mathbf{ZDZ}^H = \sum_{k = 1}^K d_k \mathbf{z}_k \mathbf{z}_k^H $, and $\mathbf{W} = \sum_{k = 1}^K c_k^2 d_k^{-1} \mathbf{x}_k \mathbf{x}_k^H$ for any $d_k > 0$, Then
\begin{equation}
\begin{aligned}
\left[                 
  \begin{array}{cc}   
   \mathrm{Toep}(\mathbf{u}) & \mathbf{\widetilde{Y}} \\  
    \mathbf{\widetilde{Y}}^H & \mathbf{W} \\  
  \end{array}
\right] &= \sum_{k = 1}^K d_k \left[                 
  \begin{array}{cc}   
    \mathbf{z}_k \\  
    c_k d_k^{-1}\mathbf{x}_k\\  
  \end{array}
\right] \left[                 
  \begin{array}{cc}   
    \mathbf{z}_k \\  
    c_k d_k^{-1}\mathbf{x}_k\\  
  \end{array}
\right]^H \\
&= \sum_{k = 1}^K  \left[                 
  \begin{array}{cc}   
    d_k \mathbf{z}_k \mathbf{z}_k^H  & c_k \mathbf{z}_k \mathbf{x}_k^H\\  
    c_k \mathbf{x}_k \mathbf{z}_k^H & c_k^2 d_k^{-1}\mathbf{x}_k \mathbf{x}_k^H \\  
  \end{array}
\right] \succeq 0
\end{aligned}
\end{equation}
% and 
% \begin{equation}
%     \mathcal{R}(\widetilde{\mathbf{Y}}) = \sum_{k = 1}^K \mathbf{A}(w) \varoast \mathbf{x}_w^T = \mathbf{Y},
% \end{equation}
which indicates that $(\mathbf{W}, \mathbf{u})$ constructed above is a feasible solution of \eqref{rank_min}. The optimality of $\mathbf{u}^*$ leads to $r^* = \mathrm{rank}(\mathrm{Toep}(\mathbf{u}^*)) \leq \mathrm{rank}(\mathrm{Toep}(\mathbf{u})) \leq K  = s$.

We next show $s \leq r^*$. Since $\mathrm{rank}(\mathrm{Toep}(\mathbf{u}^*)) = r^*$, we have the Vandermonde decomposition of $\mathrm{Toep}(\mathbf{u}^*)$
\begin{equation}
    \mathrm{Toep}(\mathbf{u}^*) = \sum_{k = 1}^{r^*} d_k \mathbf{z}_k \mathbf{z}_k^H = \mathbf{ZDZ}^H.
\end{equation}

Since $\left[                 
  \begin{array}{cc}   
    \mathrm{Toep}(\mathbf{u}^*) & \mathbf{\widetilde{Y}} \\  
    \mathbf{\widetilde{Y}}^H & \mathbf{W} \\  
  \end{array}
\right] = \left[                 
  \begin{array}{cc}   
    \mathbf{ZDZ}^H & \mathbf{\widetilde{Y}} \\  
    \mathbf{\widetilde{Y}}^H & \mathbf{W} \\  
  \end{array}
\right] \succeq 0$, based on Schur complement condition, we have $\mathbf{\widetilde{Y}} = \mathrm{Toep}(\mathbf{u}^*) \mathrm{Toep}(\mathbf{u}^*)^{+}\mathbf{\widetilde{Y}} $ ($ \mathrm{Toep}(\mathbf{u}^*)^{+}$ is the Moore–Penrose inverse of $\mathrm{Toep}(\mathbf{u}^*)$).  Hence,  $\mathrm{rank}(\mathbf{\widetilde{Y}}) \leq \mathrm{rank}(\mathrm{Toep}(\mathbf{u}^*)) = r^*$  (i.e.,$\mathbf{\widetilde{Y}}$ can be expressed as a linear combination of no more than $r^*$ atoms). Note $\|\mathbf{\widetilde{Y}} \|_{\mathcal{A}, 0} = s$ is defined as the minimum number of linear combination terms, and therefore $s \leq r^*$.
$\hfill\square$ \\

%In addition, it offers us a new way to interpret \eqref{ssdp_fast_smv}. In \eqref{ssdp_fast_smv}, $\mathbf{\widetilde{Y}}$ is an optimization variable and the program is searching for the $\mathbf{\widetilde{Y}}$ that has the smallest atomic $\ell_0$ norm while satisfying the data-consistency constraint (i.e., $\mathbf{Y} = \mathcal{R}_1(\widetilde{\mathbf{Y}})$).
